UADB: Unsupervised Anomaly Detection Booster

Unsupervised Anomaly Detection (UAD) is a key data mining problem owing to its wide real-world applications. Due to the complete absence of supervision signals, UAD methods rely on implicit assumptions about anomalous patterns (e.g., scattered/sparsely/densely clustered) to detect anomalies. However, real-world data are complex and vary significantly across different domains. No single assumption can describe such complexity and be valid in all scenarios. This is also confirmed by recent research that shows no UAD method is omnipotent. Based on above observations, instead of searching for a magic universal winner assumption, we seek to design a general UAD Booster (UADB) that empowers any UAD models with adaptability to different data. This is a challenging task given the heterogeneous model structures and assumptions adopted by existing UAD methods. To achieve this, we dive deep into the UAD problem and find that compared to normal data, anomalies (i) lack clear structure/pattern in feature space, thus (ii) harder to learn by model without a suitable assumption, and finally, leads to (iii) high variance between different learners. In light of these findings, we propose to (i) distill the knowledge of the source UAD model to an imitation learner (booster) that holds no data assumption, then (ii) exploit the variance between them to perform automatic correction, and thus (iii) improve the booster over the original UAD model. We use a neural network as the booster for its strong expressive power as a universal approximator and ability to perform flexible post-hoc tuning. Note that UADB is a model-agnostic framework that can enhance heterogeneous UAD models in a unified way. Extensive experiments on over 80 tabular datasets demonstrate the effectiveness of UADB.

==> sections/experiment.tex <==
\section{Experiments \& Analysis}
\label{sec:experiment}

In this section, we conduct comprehensive experiments to validate the effectiveness of the proposed \method framework.
We first introduce the included 14 mainstream UAD models and 84 heterogeneous real-world datasets.
Based on them, we then present the empirical results and corresponding analysis.
An ablation study is included to verify the contribution of the automatic error correction mechanism.
Finally, we visualize the results on synthetic datasets to intuitively demonstrate how UADB improves over source UAD models.
% In this section, we present the results of our experimental study on 84 real-world widely used tabular datasets. 
% We also conduct ablation study to verify the effectiveness of the proposed \method framework.
% In addition, to help better understand the effects of automatic correction mechanism, we also show some visualizations on synthetic datasets.

\subsection{Experiment Setup Details.}
% \subsection{Source Unsupervised Anomaly Detection Models}
\textbf{Source UAD Models.}
\label{sec:mainstream UAD}
As the UADB is a model-agnostic framework, we include 14 mainstream UAD techniques to test UADB's applicability and effectiveness to different UAD models with diverse architecture.
These UAD algorithms include:
\begin{enumerate}[leftmargin=*]
    \item Isolation Forest (IForest) \cite{liu2008isolation} that isolates observations by randomly selecting a feature and a splitting point.
    \item Histogram-based outlier detection (HBOS) \cite{goldstein2012histogram} assumes the feature independence and calculates the degree of outlyingness by building histograms; 
    \item Local Outlier Factor (LOF) \cite{breunig2000lof} measures the local deviation of the density of a sample with respect to its neighbors;
    \item K-Nearest Neighbors (KNN) \cite{ramaswamy2000efficient} views an instance's distance to its kth nearest neighbor as the outlying score;
    \item Principal Component Analysis (PCA) \cite{shyu2003novel} is a linear dimensionality reduction using Singular Value Decomposition of the data to project it to a lower dimensional space. In anomaly detection, it projects the data to the lower dimensional space and then reconstruct it, thus the reconstruction errors are viewed as the anomaly scores;
    \item One-class SVM (OCSVM) \cite{scholkopf1999support} maximizes the margin between the abnormal and the normal samples, and uses the hyperplane that determines the margin for decision;
    \item Clustering Based Local Outlier Factor (CBLOF) \cite{he2003discovering} classifies the samples into small clusters and large clusters  and then using the distance among clusters as anomaly scores;
    \item Connectivity-Based Outlier Factor (COF) \cite{tang2002enhancing} uses the ratio of average chaining distance of data point and the average of average chaining distance of k nearest neighbor of the data point, as the outlier score for observations;
    \item Subspace Outlier Detection (SOD) \cite{kriegel2009outlier} detects outlier in varying subspaces of a high dimensional feature space;
    \item Empirical-Cumulative-distribution-based Outlier Detection (ECOD) \cite{li2022ecod} is a parameter-free, highly interpretable outlier detection algorithm based on empirical CDF functions;
    \item Gaussian Mixture Models (GMM) \cite{reynolds2009gaussian} fit k Gaussians to the data. Then for each data point, calculate the probabilities of belonging to each of the clusters, where the lower probabilities indicate higher anomaly scores;
    \item Lightweight on-line detector of anomalies (LODA) \cite{pevny2016loda} is an ensemble detector and is particularly useful in domains where a large number of samples need to be processed in real-time or in domains where the data stream is subject to concept drift and the detector needs to be updated online;
    \item Copula Based Outlier Detector (COPOD) \cite{li2020copod} is a parameter-free, highly interpretable outlier detection algorithm based on empirical copula models;
    \item Deep Support Vector Data Description (DeepSVDD) \cite{ruff2018deep} trains a neural network while minimizing the volume of a hypersphere that encloses the network representations of the data, the distance of the transformed embedding to the hypersphere's center is used to calculate the anomaly score.
\end{enumerate}

The aforementioned 14 UAD methods are widely used in practice and vary significantly in terms of both methodologies (e.g., neighbor-based~\cite{breunig2000lof,tang2002enhancing,ramaswamy2000efficient}, clustering-based~\cite{reynolds2009gaussian,he2003discovering}, density-based~\cite{goldstein2012histogram,li2022ecod}) and model architectures (e.g., tree~\cite{liu2008isolation}, support vector machine~\cite{scholkopf1999support}, neural network~\cite{ruff2018deep}).
Thus they can be used to perform a comprehensive test of the effectiveness of and applicability of UADB.

% (1) Isolation Forest (IForest) \cite{liu2008isolation} isolates observations by randomly selecting a feature and then randomly selecting a split value between the maximum and minimum values of the selected feature; (2) Histogram-based outlier detection (HBOS) \cite{goldstein2012histogram} assumes the feature independence and calculates the degree of outlyingness by building histograms; (3) Local Outlier Factor (LOF) \cite{breunig2000lof} measures the local deviation of the density of a given sample with respect to its neighbors; (4) K-Nearest Neighbors (KNN) \cite{ramaswamy2000efficient} views an instance's distance to its kth nearest neighbor as the outlying score; 
% (5) Principal Component Analysis (PCA) \cite{shyu2003novel} is a linear dimensionality reduction using Singular Value Decomposition of the data to project it to a lower dimensional space. In anomaly detection, it projects the data to the lower dimensional space and then reconstruct it, thus the reconstruction errors are viewed as the anomaly scores; (6) One-class SVM (OCSVM) \cite{scholkopf1999support} maximizes the margin between the abnormal and the normal samples, and defines the decision boundary as the hyperplane that determines the margin; (7) Clustering Based Local Outlier Factor (CBLOF) \cite{he2003discovering} classifies the samples into small clusters and large clusters  and then using the distance among clusters as anomaly scores; (8) Connectivity-Based Outlier Factor (COF) \cite{tang2002enhancing} uses the ratio of average chaining distance of data point and the average of average chaining distance of k nearest neighbor of the data point, as the outlier score for observations; (9) Subspace Outlier Detection (SOD) \cite{kriegel2009outlier} aims to detect outlier in varying subspaces of a high dimensional feature space; (10) Empirical-Cumulative-distribution-based Outlier Detection (ECOD) \cite{li2022ecod} is a parameter-free, highly interpretable outlier detection algorithm based on empirical CDF functions; (11) Gaussian Mixture Models (GMM) \cite{reynolds2009gaussian} fit k Gaussians to the data. Then for each data point, calculate the probabilities of belonging to each of the clusters, where the lower probabilities indicate higher anomaly scores; (12) Lightweight on-line detector of anomalies (LODA) \cite{pevny2016loda} is an ensemble detector and is particularly useful in domains where a large number of samples need to be processed in real-time or in domains where the data stream is subject to concept drift and the detector needs to be updated on-line; (13) Copula Based Outlier Detector (COPOD) \cite{li2020copod} is a parameter-free, highly interpretable outlier detection algorithm based on empirical copula models; (14) Deep Support Vector Data Description (DeepSVDD) \cite{ruff2018deep} trains a neural network while minimizing the volume of a hypersphere that encloses the network representations of the data, and the distance of the transformed embedding to the hypersphere's center is used to calculate the anomaly score.


% (14) Deep Autoencoding Gaussian Mixture Model (DAGMM) \cite{zong2018deep} utilizes a deep autoencoder to generate a low-dimensional representation and reconstruction error for each input data point, which is further fed into a Gaussian Mixture Model (GMM).

% The above original mainstream UAD methods are used as source models (teacher).
% Given any source model, we aim to train a target booster (student) to enhance the prediction performance over this source model.
% During the cascade training procedure of target booster, the parameters of source models are fixed.
% We only use the output of booster at the final iteration as the predictive anomaly score.
% All these designs make \method be a model-agnostic framework, and we will further demonstrate the effectiveness of \method in the following sections.



% \subsection{Experiments on Real-world Datasets}
% \subsubsection{Data settings}
\textbf{Real-world Datasets.}
As described before, UAD on tabular datasets are challenging due to the heterogeneity, complexity, and diversity of tabular data.
Table~\ref{tab:datasets} shows the statistics of the 84 heterogeneous tabular datasets that are included for a comprehensive evaluation.
Note that, in addition to the native tabular datasets (i.e., from abalone to yeast), datasets from larger and high-dimensional CV and NLP tasks are also included.
However, as many UAD models such as IForest \cite{liu2008isolation} and OCSVM \cite{scholkopf1999support} cannot directly handle CV or NLP task, we follow previous work \cite{han2022adbench} and use a CV/NLP feature extractor to generate tabular versions of these datasets.
These datasets vary significantly in properties and application domains, including health care (e.g., disease diagnosis), finance (e.g. credit card fraud detection), image processing (e.g. object identification), language processing (e.g. speech recognition) and more.


% Unlike large and high-dimensional CV and NLP tasks, traditional tabular UAD tasks are relatively small \cite{campos2016evaluation, emmott2015meta, pang2021deep}.
% To verify the effectiveness of \method on complex tasks and enrich the application domains of \method, we introduce some complex datasets from CV and NLP domains.
% However, some traditional UAD models such as OCSVM \cite{scholkopf1999support} cannot directly run on CV or NLP tasks.
% Therefore, following previous work \cite{han2022adbench}, we extract features from CV and NLP tasks to generate tabular versions of them.
% In this paper, we used more than 80 widely used tabular datasets to validate the broad applicability of \method.
% These datasets cover various application domains, including health care (e.g., disease diagnosis), finance (e.g. credit card fraud detection), image processing (e.g. object identification), language processing (e.g. speech recognition) and more.
% Table \ref{tab:datasets} lists the anomaly ratio and application domains of the 84 datasets.
% Among all datasets, \textit{CIFAR10, FashionMNIST, SVHN} and \textit{agnews} are multi-classes tasks.
% For every class of the multi-classes, we set this class as normal and downsample the remaining classes to 5\% of the total instances as
% anomalies by default.

\textbf{UADB Setup.}
As mentioned before, UADB adopt a neural network as the booster model for its strong expressive power as a universal approximator and ability to perform flexible post-hoc tuning.
Since the source UAD models $f_T(\cdot)$ are usually not incrementally learnable (e.g.,~\cite{liu2008isolation,scholkopf1999support}), we only optimize and keep the booster $f_B(\cdot;\theta)$ as the final UAD model.
Specifically, the booster model is a simple 3-layer fully-connected MLP (Multi-layer Perceptron) with 128 neurons in each hidden layer.
In $t$-th training step/iteration of UADB, the booster $f_B(\cdot;\theta)$ is updated w.r.t objective $argmin_\theta\mathcal{L}(f_B(\textbf{X};\theta), \hat{\textbf{y}}^{(t)})$ for 10 epochs with batch size set to 256, and the total number of UADB training steps $T=10$.

\textbf{Evaluation Metric \& Implementation Details.}
Following the common practice of previous works, we use \textit{Area Under the Curve of Receiver Characteristic Operator} (AUCROC) and \textit{Average Precision} (AP) to evaluate UAD models' performance.
Larger AUCROC/AP score indicates better detection performance.
We use the popular PyOD Python package~\cite{zhao2019pyod} to implement all source UAD models, and apply their default parameter settings in PyOD\footnote{Please refer to \url{https://pyod.readthedocs.io/en/latest/pyod.models.html}.}.
The booster model is implemented using the PyTorch~\cite{paszke2019pytorch} framework.

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.85\linewidth]{pictures/decision_boundary.pdf}
% \caption{
% Visualization of the detection results of UAD models and their UADB boosters when facing different types of anomalies.
% Specifically, we generate 4 synthetic datasets (in 4 rows) with different types of anomalies, i.e. Clustered, Global, Local and Dependency.
% For each dataset, we test two UAD models (1st \& 3rd columns) that are best in handling the corresponding anomaly~\cite{han2022adbench} and their boosters (2nd \& 4th columns), we then plot their decision boundaries.
% In each figure, the orange/blue interface represents the normal/abnormal space predicted by the model.
% We can observe that UADB boosters can maintain the right decisions of the source model by knowledge transfer, while correcting the wrong predictions by adaptive error correction.
% UADB improves the UAD model's detection results on all 8 model-anomaly-type pairs, achieving up to 86\% correction rate.
% % The process of change of decision boundary on different types of anomalies.
% % The accuracy errors are also reported.
% % Here, we use synthetic dataset to 4 types of anomalies, i.e. Clustered, Global, Local and Dependency.
% % Each type of anomaly is presented in one row.
% % For each UAD on a specific synthetic dataset, we visualize the original (teacher's) decision boundary and its booster's decision boundary (at final iteration) respectively (in pairs).
% % The blue interface represents the abnormal space, and the darker the color is, the higher the anomaly scores are.
% % The orange interface represents the normal space.
% % The red dotted line represents the learned decision boundary.
% % It is clear that \method could improve accuracy in all settings.
% % For the samples that teacher has made right conclusions, booster could maintain the conclusions for majority of them.
% % For the incorrect conclusions made by teacher, booster has the ability to correct most of them.
% % For example, on synthetic data with clustered anomalies, teacher's decision normal space (orange) contains a group of outliers.
% % Surprisingly, booster's decision boundary was changed a lot by exploiting correction mechanism, thus the group of outliers were removed from normal space. 
% }
% \label{fig:decision_boundary}
% \end{figure*}


% \subsubsection{Experimental details.}
% As mentioned above, the target booster should be capable to boost any source UAD algorithm.
% Here, we adopt a Multilayer Perceptron (MLP) as the booster for its strong expressive power as a universal function approximator, and also for its ability to perform flexible post-hoc tuning.
% For the above mentioned unsupervised AD algorithms in Section \ref{sec:mainstream UAD}, we use their default hyperparameter settings~\footnote{We refer to the parameter settings of original repositories. See \url{https://pyod.readthedocs.io/en/latest/pyod.models.html} for more details.}.
% We evaluate the \method's performance by two widely used metrics in AD: AUCROC (Area Under Receiver Operating Characteristic Curve) and AP (Average Precision).
% Larger AUCROC/AP indicates better performance.
% The booster is a cascade model with multiple training iterations, in this paper, the total number of iterations is set to 10.


\begin{figure*}[t]
\centering
\includegraphics[width=0.85\linewidth]{pictures/decision_boundary.pdf}
\caption{
Visualization of the detection results of UAD models and their UADB boosters when facing different types of anomalies.
Specifically, we generate 4 synthetic datasets (in 4 rows) with different types of anomalies, i.e. Clustered, Global, Local and Dependency.
For each dataset, we test two UAD models (1st \& 3rd columns) that are best in handling the corresponding anomaly~\cite{han2022adbench} and their boosters (2nd \& 4th columns), we then plot their decision boundaries.
In each figure, the orange/blue interface represents the normal/abnormal space predicted by the model.
We can observe that UADB boosters can maintain the right decisions of the source model by knowledge transfer, while correcting the wrong predictions by adaptive error correction.
UADB improves the UAD model's detection results on all 8 model-anomaly-type pairs, achieving up to 86\% correction rate.
}
\label{fig:decision_boundary}
\end{figure*}


\subsection{Visualization on Synthetic Datasets}
\label{sec:main results}



\subsection{Results \& Analysis on Real-world Datasets}
\label{sec:main results}

\textbf{UADB Improvements.}




Recent comprehensive studies \cite{han2022adbench, gopalan2019pidforest} have demonstrated that anomaly types in real world applications could be roughly divided into four specific types, i.e. clustered anomalies, global anomalies, local anomalies and dependency anomalies.
Please see Fig. \ref{fig:decision_boundary} for more details of the four types of outliers.
% Fig. \ref{} shows the 2-d visualization of the four types of outliers.
Among aforementioned 14 mainstream UAD algorithms, IForest performs well on the four anomaly types, HBOS performs well on clustered and global anomalies, LOF performs well on local anomalies, and KNN performs well on dependency anomalies \cite{han2022adbench}.
We first select the 4 representative UAD algorithms and show the boosted performance over them in Table \ref{tab:results with multiple iterations}.
From the listed datatsets, the \method outperforms all source UAD models in all settings.
For most cases, the predictive accuracy of \method gradually increases through multiple iterations.
Even for the cases that the booster's accuracy is lower than teacher at early iterations (e.g. \method's performance over IForest on \textit{skin} in Table \ref{tab:results with multiple iterations}.(a)), booster's performance would gradually surpass the teacher during subsequent iterations.
Furthermore, \method yields surprisingly improvements over LOF on \textit{http}, where the booster obtains improvements over 60\% and 90\% on AUCROC and AP respectively.
\method also obtains huge improvements over LOF on \textit{shuttle, satimage-2, optdigits}, and also over KNN on \textit{shuttle, satimage-2}.
This indicates that \method has the possibility to enhance the teacher's unsatisfactory performance.

Since our work verifies the effectiveness of \method on 14 mainstream UAD algorithms on 84 datasets, the length of the article limits us to show 14 * 84 results in detail.
Therefore, we statistically summarize the remaining experiments in Table \ref{tab:results_statistic} and Fig \ref{fig:box overall}.
We can observe that on average, \method improves the performance of all mainstream UAD algorithms in all settings, which reveals that \method is a model-agnostic framework.
In addition, for each UAD algorithms, \method enhances the performance on over 55\% of datasets in terms of AUCROC, and on over 61\% of datasets in terms of AP.
Furthermore, LOF, COF, SOD and DeepSVDD's average improvements even exceed 0.05 in terms of both AUCROC and AP.
As mentioned above, IForest performs relatively well under different anomaly types \cite{han202adbench}.
We could find that in our settings, \method could still enhance the performance of IForest on a large proportion of datasets, which demonstrated the strong ability of \method.
Previous studies indicated \cite{han2022adbench} that without the guidance of label information, DL-based unsupervised algorithms are harder to train (due to more hyperparameters) and more difficult to tune hyperparameters, leading to unsatisfactory performance.
This lead to some observations that some DL-based unsupervised methods like DeepSVDD are surprisingly worse than shallow methods.
However, in our settings, \method obtained a surprisingly improvement over DeepSVDD.
We argue that though without true labels, DL-based UAD could not achieve satisfactory performance, \method could still leverages the prior knowledge from teacher and variance between teacher and booster to perform automatic correction, and thus enhance the performance.

% \subsubsection{Correction visualization (ranking figure)}
\subsubsection{Ablation Study}
In this section, to further verify the contribution of \method framework, we conduct ablation study.
\method is a model-agnostic framework and the booster is improved by automatic error correction.
The automatic correction mechanism is performed by ingeniously utilizing the variance between booster and source UAD model.
Therefore, we consider following 5 variants and \method to demonstrate the effectiveness of \method.

\begin{itemize}
\item 
Origin: the origin represents the source unsupervised AD.
\item
SUDO\_booster: only use the source model's output to supervise the training process of the booster, which means that there is only one iteration and the booster's output are used as predictive anomaly score at inference.
\item
Discrepancy\_booster: only use the source model's output to supervise the training process of the booster, which means that there is only one iteration.
At inference, using the discrepancy (Standard deviation) between booster's output and source model's output as predictive anomaly score.
\item
C\_sudo\_booster: this is a cascade SUDO\_booster. 
During the training process, the variance between booster and source model's outputs is not added to the pseudo labels.
Specifically, after MinMax Normalization, booster's output at each iteration is directly used as next iteration's training label (the variance will be added to pseudo labels for the training process of \method).
At inference, booster's output at final iteration is used as predictive anomaly score.
\item
C\_discrepancy\_booster: this is a cascade Discrepancy\_booster. 
The training process is the same as C\_sudo\_booster, however, at inference, the discrepancy (Standard deviation) between booster's output at final iteration and source model's output would be used as predictive anomaly score.
\end{itemize}

The ablation results are shown in Table \ref{tab:ablation study}.
From Table \ref{tab:ablation study}, it is clear that \method is the best performer.
\method outperforms C\_sudo\_booster and C\_discrepancy\_booster by a large margin, which indicates that introducing the variance between booster and source model into pseudo labels could automatically correct some errors, thereby enhance the performance of booster.
In addition, on average, C\_sudo\_booster's performance is better than SUDO\_booster's performance, and also C\_discrepancy\_booster is better than Discrepancy\_booster.
We assume that during multiple iterations, the booster may ignore some overfitted samples.

% \subsubsection{Robustness}
\subsection{Extensive experiments on Synthetic Datasets}
To better understand the effect of automatic correction mechanism, we design to present visualizations on different anomaly types of synthetic dastasets to show \method's influence on the evolution of target model's decision boundaries.
As mentioned in Section \ref{sec:main results}, anomalies could be roughly divided into 4 types, i.e. clustered anomalies, global anomalies, local anomalies, and dependency anomalies.
We first generate 4 synthetic datasets, where each dataset has 300 two-dimensional samples (anomaly rate: 15\%).
The outliers are generated by Normal distribution in all settings.
As for outliers, (i) clustered anomalies are also generated by Normal distribution, we control the distance between clustered anomalies and inliers to ensure anomalies are deviant from the majority. 
The clustered anomalies are far away from the normal instances;
(ii) global anomalies are generated from Uniform distribution, so the anomalies will be evenly distributed in 2d space; 
(iii) local anomalies are generated by Normal distribution which are well overlapped with the normal samples, however, we control the covariance so that they are deviant from their local neighborhoods;
(iv) dependency anomalies are samples that are inconsistent with the dependency structure of normal data.
Please see Fig. \ref{fig:decision_boundary} for more details.

Recall Section \ref{sec:main results}, we mentioned that IForest performs well on the four anomaly types, HBOS performs well on clustered and global anomalies, LOF performs well on local anomalies, and KNN performs well on Dependency anomalies \cite{han2022adbench}.
Due to the limitation of space, we show \method's performance over IForest and HBOS on clusterd dataset (i.e. anomaly type in the synthetic data is clustered), IForest and HBOS on global dataset, IForest and LOF on local dataset, IForest and KNN on dependency dataset, which is presented in Fig \ref{fig:decision_boundary}.


\begin{table*}[t]
\scriptsize
\centering
\caption{Data description of the 84 real-world datasets.}
\label{tab:datasets}
\setlength{\tabcolsep}{0.5mm}{
\begin{tabular}{ccc|ccc|ccc|ccc} 
\toprule
\textbf{Datasets}         & \textbf{\% Anomaly} & \textbf{Category} & \textbf{Datasets}    & \textbf{\% Anomaly} & \textbf{Category} & \textbf{Datasets}        & \textbf{\% Anomaly} & \textbf{Category} & \textbf{Datasets}        & \textbf{\% Anomaly} & \textbf{Category}  \\ 
\midrule
\textbf{abalone}          & 49.82               & Biology           & \textbf{mammography} & 2.32                & Healthcare        & \textbf{WDBC}            & 2.72                & Healthcare        & \textbf{FashionMNIST\_6} & 5.00                & Image              \\
\textbf{ALOI}             & 3.04                & Image             & \textbf{mnist}       & 9.21                & Image             & \textbf{Wilt}            & 5.33                & Botany            & \textbf{FashionMNIST\_7} & 5.00                & Image              \\
\textbf{annthyroid}       & 7.42                & Healthcare        & \textbf{musk}        & 3.17                & Chemistry         & \textbf{wine}            & 7.75                & Chemistry         & \textbf{FashionMNIST\_8} & 5.00                & Image              \\
\textbf{Arrhythmia}       & 45.78               & Healthcare        & \textbf{optdigits}   & 2.88                & Image             & \textbf{WPBC}            & 23.74               & Healthcare        & \textbf{FashionMNIST\_9} & 5.00                & Image              \\
\textbf{breastw}          & 34.99               & Healthcare        & \textbf{PageBlocks}  & 9.46                & Document          & \textbf{yeast}           & 34.16               & Biology           & \textbf{SVHN\_0}         & 5.00                & Image              \\
\textbf{cardio}           & 9.61                & Healthcare        & \textbf{Parkinson}   & 75.38               & Healthcare        & \textbf{CIFAR10\_0}      & 5.00                & Image             & \textbf{SVHN\_1}         & 5.00                & Image              \\
\textbf{Cardiotocography} & 22.04               & Healthcare        & \textbf{pendigits}   & 2.27                & Image             & \textbf{CIFAR10\_1}      & 5.00                & Image             & \textbf{SVHN\_2}         & 5.00                & Image              \\
\textbf{concrete}         & 50.00               & Physical          & \textbf{Pima}        & 34.90               & Healthcare        & \textbf{CIFAR10\_2}      & 5.00                & Image             & \textbf{SVHN\_3}         & 5.00                & Image              \\
\textbf{cover}            & 0.96                & Botany            & \textbf{satellite}   & 31.64               & Astronautics      & \textbf{CIFAR10\_3}      & 5.00                & Image             & \textbf{SVHN\_4}         & 5.00                & Image              \\
\textbf{fault}            & 34.67               & Physical          & \textbf{satimage-2}  & 1.22                & Astronautics      & \textbf{CIFAR10\_4}      & 5.00                & Image             & \textbf{SVHN\_5}         & 5.00                & Image              \\
\textbf{glass}            & 4.21                & Forensic          & \textbf{shuttle}     & 7.15                & Astronautics      & \textbf{CIFAR10\_5}      & 5.00                & Image             & \textbf{SVHN\_6}         & 5.00                & Image              \\
\textbf{HeartDisease}     & 44.44               & Healthcare        & \textbf{skin}        & 20.75               & Image             & \textbf{CIFAR10\_6}      & 5.00                & Image             & \textbf{SVHN\_7}         & 5.00                & Image              \\
\textbf{Hepatitis}        & 16.25               & Healthcare        & \textbf{smtp}        & 0.03                & Web               & \textbf{CIFAR10\_7}      & 5.00                & Image             & \textbf{SVHN\_8}         & 5.00                & Image              \\
\textbf{http}             & 0.39                & Web               & \textbf{SpamBase}    & 39.91               & Document          & \textbf{CIFAR10\_8}      & 5.00                & Image             & \textbf{SVHN\_9}         & 5.00                & Image              \\
\textbf{imgseg}           & 42.86               & image             & \textbf{speech}      & 1.65                & Linguistics       & \textbf{CIFAR10\_9}      & 5.00                & Image             & \textbf{agnews\_0}       & 5.00                & NLP                \\
\textbf{InternetAds}      & 18.72               & Image             & \textbf{Stamps}      & 9.12                & Document          & \textbf{FashionMNIST\_0} & 5.00                & Image             & \textbf{agnews\_1}       & 5.00                & NLP                \\
\textbf{Ionosphere}       & 35.90               & Oryctognosy       & \textbf{thyroid}     & 2.47                & Healthcare        & \textbf{FashionMNIST\_1} & 5.00                & Image             & \textbf{agnews\_2}       & 5.00                & NLP                \\
\textbf{landsat}          & 20.71               & Astronautics      & \textbf{vertebral}   & 12.50               & Biology           & \textbf{FashionMNIST\_2} & 5.00                & Image             & \textbf{agnews\_3}       & 5.00                & NLP                \\
\textbf{letter}           & 6.25                & Image             & \textbf{vowels}      & 3.43                & Linguistics       & \textbf{FashionMNIST\_3} & 5.00                & Image             & \textbf{amazon}          & 5.00                & NLP                \\
\textbf{Lymphography}     & 4.05                & Healthcare        & \textbf{Waveform}    & 2.90                & Physics           & \textbf{FashionMNIST\_4} & 5.00                & Image             & \textbf{imdb}            & 5.00                & NLP                \\
\textbf{magic.gamma}      & 35.16               & Physical          & \textbf{WBC}         & 4.48                & Healthcare        & \textbf{FashionMNIST\_5} & 5.00                & Image             & \textbf{yelp}            & 5.00                & NLP                \\
\bottomrule
\end{tabular}}
\end{table*}


\begin{table*}[t!]
\footnotesize
\centering
\caption{
The detection performance improvement achieved by UADB over 14 source UAD models on 84 datasets.
``Original'' indicates the average score achieved by the corresponding source UAD model on all datasets.
``Improvement'' indicates the average score improvement achieved by the UADB booster of the UAD model.
``Effects'' represents the number of datasets that UADB booster made improvements over the source model.
% The statistic information of all mainstream unsupervised AD methods' results on 84 datasets.
% The orginal means UAD's average performance in terms of AUCROC/AP over all datasets.
% For each UAD, AUCROC/AP improvements (\method - teacher) averaged over all datasets are reported.
% The effects represent the number of datasets which \method has made improvements over teacher.
}
\label{tab:results_statistic}
\setlength{\tabcolsep}{0.9mm}{
\begin{tabular}{c|c|cccccccccccccc} 
\toprule
\multicolumn{2}{c|}{\textbf{Source UAD Model}}                 & \textbf{IForest} & \textbf{\textbf{HBOS}} & \textbf{LOF} & \textbf{KNN} & \textbf{\textbf{PCA}} & \textbf{OCSVM} & \textbf{CBLOF} & \textbf{COF} & \textbf{SOD} & \textbf{ECOD} & \textbf{\textbf{GMM}} & \textbf{LODA} & \textbf{COPOD} & \textbf{\textbf{DeepSVDD}}  \\ 
\midrule
\multirow{4}{*}{\textbf{AUCROC}} & \textbf{Original}    & 0.7028           & 0.6848                 & 0.6311       & 0.6794       & 0.6930                & 0.6750         & 0.7110         & 0.6105       & 0.6638       & 0.6866        & 0.7274                & 0.6571        & 0.6882         & 0.5346                      \\ 
\cmidrule{2-16}
                                  & \textbf{Improvement} & 0.0117           & 0.0153                 & 0.0694       & 0.0452       & 0.0130                & 0.0241         & 0.0215         & 0.0580       & 0.0562       & 0.0144        & 0.0133                & 0.0293        & 0.0116         & 0.0979                      \\ 
\cmidrule{2-16}
                                  & \textbf{Effects}     & 49               & 59                     & 51           & 46           & 53                    & 58             & 51             & 57           & 57           & 57            & 47                    & 62            & 52             & 68                          \\ 
\midrule
\multirow{4}{*}{\textbf{AP }}     & \textbf{Original}    & 0.3012           & 0.2918                 & 0.1903       & 0.2550       & 0.3051                & 0.2738         & 0.3057         & 0.1989       & 0.2322       & 0.2908        & 0.2805                & 0.2636        & 0.2832         & 0.1727                      \\ 
\cmidrule{2-16}
                                  & \textbf{Improvement} & 0.0134           & 0.0137                 & 0.1146       & 0.0627       & 0.0010                & 0.0229         & 0.0184         & 0.0670       & 0.0742       & 0.0101        & 0.0283                & 0.0390        & 0.0146         & 0.0741                      \\ 
\cmidrule{2-16}
                                  & \textbf{Effects}     & 57               & 62                     & 56           & 51           & 62                    & 59             & 57             & 60           & 60           & 66            & 51                    & 64            & 64             & 70                          \\
\bottomrule
\end{tabular}}
\end{table*}

\begin{table*}[t!]
\footnotesize
\centering
\caption{Ablation study results. The average AUCROC and AP over 84 datasets are reported. For each UAD model, we show the results of 6 variants (UAD itself and 5 different types of booster). The best results are highlighted in bold.}
\label{tab:ablation study}
\setlength{\tabcolsep}{0.7mm}{
\begin{tabular}{c|cccccccccccccc|c} 
\toprule
\multicolumn{16}{c}{\textbf{Comparison between different booster training strategies in terms of AUCROC}} \\ 
\midrule
\textbf{Source UAD Model}                 & \textbf{Iforest}          & \textbf{HBOS}          & \textbf{LOF}          & \textbf{KNN}          & \textbf{PCA}          & \textbf{OCSVM}          & \textbf{CBLOF}          & \textbf{COF}          & \textbf{SOD}          & \textbf{ECOD}          & \textbf{\textbf{GMM}}                   & \textbf{LODA}          & \textbf{COPOD}          & \textbf{\textbf{DeepSVDD}} & \textbf{Average}  \\ 
\midrule
\textbf{Origin}                  & 0.7028                    & 0.6848                 & 0.6311                & 0.6794                & 0.6930                & 0.6750                  & 0.7110                  & 0.6105                & 0.6638                & 0.6866                 & 0.7274                                  & 0.6571                 & 0.6882                  & 0.5346                     & 0.6777            \\ 
\hline
\textbf{SUDO\_booster}           & 0.6896                    & 0.6728                 & 0.6365                & 0.6778                & 0.6943                & 0.6733                  & 0.7093                  & 0.6108                & 0.6813                & 0.6863                 & 0.7173                                  & 0.6751                 & 0.6713                  & 0.5641                     & 0.6766            \\ 
\hline
\textbf{Discrepancy\_booster}    & 0.5589                    & 0.5526                 & 0.5807                & 0.5850                & 0.6065                & 0.6019                  & 0.5356                  & 0.5439                & 0.6025                & 0.5497                 & 0.6362                                  & 0.5677                 & 0.5607                  & 0.5851                     & 0.5755            \\ 
\hline
\textbf{C\_sudo\_booster}        & 0.6838                    & 0.6688                 & 0.6334                & 0.6686                & 0.6809                & 0.6618                  & 0.7008                  & 0.6073                & 0.6701                & 0.6722                 & 0.7031                                  & 0.6736                 & 0.6658                  & 0.5667                     & 0.6685            \\ 
\hline
\textbf{C\_discrepancy\_booster} & 0.6235                    & 0.5904                 & 0.5731                & 0.6144                & 0.6195                & 0.5970                  & 0.5679                  & 0.5670                & 0.6358                & 0.6122                 & 0.6597                                  & 0.5761                 & 0.6039                  & 0.5580                     & 0.6031            \\ 
\hline
\textbf{UADB}                    & \textbf{0.7144}           & \textbf{0.7001}        & \textbf{0.7004}       & \textbf{0.7245}       & \textbf{0.7060}       & \textbf{0.6991}         & \textbf{0.7324}         & \textbf{0.6686}       & \textbf{0.7199}       & \textbf{0.7010}        & \textbf{\textbf{0.7407}}                & \textbf{0.6864}        & \textbf{0.6998}         & \textbf{\textbf{0.6343}}   & \textbf{0.7072}   \\ 
\bottomrule
\multicolumn{1}{l}{}             & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{}   & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{}   &                                         & \multicolumn{1}{l}{}   & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}       &                   \\ 
\toprule
\multicolumn{16}{c}{\textbf{\textbf{Comparison between different booster training strategies in terms of AUCROC}}}\\ 
\midrule
\textbf{Source UAD Model}                 & \textbf{\textbf{Iforest}} & \textbf{\textbf{HBOS}} & \textbf{\textbf{LOF}} & \textbf{\textbf{KNN}} & \textbf{\textbf{PCA}} & \textbf{\textbf{OCSVM}} & \textbf{\textbf{CBLOF}} & \textbf{\textbf{COF}} & \textbf{\textbf{SOD}} & \textbf{\textbf{ECOD}} & \textbf{\textbf{\textbf{\textbf{GMM}}}} & \textbf{\textbf{LODA}} & \textbf{\textbf{COPOD}} & \textbf{\textbf{DeepSVDD}} & \textbf{Average}  \\ 
\midrule
\textbf{Origin}                  & 0.3012                    & 0.2918                 & 0.1903                & 0.2550                & 0.3051                & 0.2738                  & 0.3057                  & 0.1989                & 0.2322                & 0.2908                 & 0.2805                                  & 0.2623                 & 0.2832                  & 0.1727                     & 0.2670            \\ 
\hline
\textbf{SUDO\_booster}           & 0.2966                    & 0.2926                 & 0.2257                & 0.2572                & 0.2923                & 0.2735                  & 0.3086                  & 0.2154                & 0.2608                & 0.2838                 & 0.2901                                  & 0.2865                 & 0.2841                  & 0.2187                     & 0.2744            \\ 
\hline
\textbf{Discrepancy\_booster}    & 0.1588                    & 0.1629                 & 0.1739                & 0.1837                & 0.1946                & 0.1854                  & 0.1580                  & 0.1647                & 0.1881                & 0.1537                 & 0.2080                                  & 0.1813                 & 0.1627                  & 0.1856                     & 0.1751            \\ 
\hline
\textbf{C\_sudo\_booster}        & 0.2946                    & 0.2911                 & 0.2127                & 0.2594                & 0.2938                & 0.2760                  & 0.3095                  & 0.2132                & 0.2647                & 0.2837                 & 0.3033                                  & 0.2887                 & 0.2817                  & 0.2132                     & 0.2748            \\ 
\hline
\textbf{C\_discrepancy\_booster} & 0.2078                    & 0.2057                 & 0.1854                & 0.2076                & 0.2255                & 0.1999                  & 0.1825                  & 0.1802                & 0.2260                & 0.1940                 & 0.2564                                  & 0.1897                 & 0.2015                  & 0.1988                     & 0.2048            \\ 
\hline
\textbf{UADB}                    & \textbf{0.3146}           & \textbf{0.3055}        & \textbf{0.3049}       & \textbf{0.3178}       & \textbf{0.3061}       & \textbf{0.2967}         & \textbf{0.3241}         & \textbf{0.2659}       & \textbf{0.3064}       & \textbf{0.3009}        & \textbf{\textbf{0.3092}}                & \textbf{0.3013}        & \textbf{0.2978}         & \textbf{\textbf{0.2468}}   & \textbf{0.3039}   \\
\bottomrule
\end{tabular}}
\end{table*}


\begin{table*}
\scriptsize
\centering
\caption{\method's performance on some representative unsupervised AD methods (teacher) in terms of AUCROC and AP (higher is better).
Due to the limited space, only 4 representative UADs on the 10 best datasets are included here.
For each method, we show the results of the best 10 datasets among over 80 datasets.
Each row represents a specific UAD's experiments in terms of AUCROC and AP
Here, the total iterations of cascade student is set to 10.
We briefly present the second, fourth, sixth, eighth, and tenth iterations.
The improvement indicates the booster's predictive anomaly score at final iteration against target model (booster's - target's). 
}
\label{tab:results with multiple iterations}
\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{c|c|ccccc|ccc|c|ccccc|c} 
\cmidrule[\heavyrulewidth]{1-8}\cmidrule[\heavyrulewidth]{10-17}
\multicolumn{8}{c}{\textbf{(a) Student’s improvement compared to Teacher (IForest) in terms of AUCROC }}                                                                  &  & \multicolumn{8}{c}{\textbf{(b) Student’s improvement compared to Teacher (IForest) in terms of AP }}                                                                       \\ 
\cmidrule{1-8}\cmidrule{10-17}
\textbf{Datasets}        & \textbf{Teacher}     & \textbf{iter 2} & \textbf{iter 4} & \textbf{iter~6} & \textbf{iter~8} & \textbf{iter 10}     & \textbf{Improvement} &  & \textbf{Datasets}        & \textbf{Teacher}     & \textbf{iter 2} & \textbf{iter~4} & \textbf{iter~6} & \textbf{iter~8} & \textbf{iter~10}     & \textbf{Improvement}  \\ 
\cmidrule{1-8}\cmidrule{10-17}
\textbf{speech}          & 0.5057               & 0.579           & 0.6002          & 0.613           & 0.62            & 0.6233               & 0.1176               &  & \textbf{pendigits}       & 0.3392               & 0.3995          & 0.4154          & 0.4505          & 0.4973          & 0.5524               & 0.2132                \\
\textbf{Wilt}            & 0.4276               & 0.4407          & 0.4989          & 0.5305          & 0.5309          & 0.5364               & 0.1088               &  & \textbf{vowels}          & 0.1825               & 0.1743          & 0.1835          & 0.2463          & 0.3143          & 0.3408               & 0.1582                \\
\textbf{satellite}       & 0.6668               & 0.6988          & 0.7117          & 0.725           & 0.7413          & 0.7625               & 0.0957               &  & \textbf{satellite}       & 0.6248               & 0.7074          & 0.7163          & 0.7252          & 0.7317          & 0.7399               & 0.1151                \\
\textbf{vowels}          & 0.8118               & 0.8318          & 0.8488          & 0.8707          & 0.8918          & 0.9066               & 0.0949               &  & \textbf{InternetAds}     & 0.5078               & 0.5166          & 0.5221          & 0.5313          & 0.5468          & 0.5588               & 0.051                 \\
\textbf{abalone}         & 0.4989               & 0.5435          & 0.5524          & 0.5589          & 0.5603          & 0.5663               & 0.0674               &  & \textbf{abalone}         & 0.5111               & 0.531           & 0.5379          & 0.5443          & 0.5468          & 0.5529               & 0.0418                \\
\textbf{SpamBase}        & 0.5997               & 0.6333          & 0.6393          & 0.6433          & 0.6461          & 0.6472               & 0.0475               &  & \textbf{wine}            & 0.1905               & 0.2051          & 0.2141          & 0.2244          & 0.2281          & 0.228                & 0.0376                \\
\textbf{skin}            & 0.6756               & 0.6705          & 0.697           & 0.7032          & 0.7127          & 0.7216               & 0.0459               &  & \textbf{Hepatitis}       & 0.2534               & 0.2702          & 0.2893          & 0.2931          & 0.2924          & 0.2892               & 0.0358                \\
\textbf{landsat}         & 0.4716               & 0.4677          & 0.4854          & 0.4962          & 0.5089          & 0.5172               & 0.0457               &  & \textbf{cardio}          & 0.4841               & 0.501           & 0.5083          & 0.5071          & 0.5125          & 0.5153               & 0.0312                \\
\textbf{InternetAds}     & 0.6988               & 0.705           & 0.7088          & 0.715           & 0.7243          & 0.7348               & 0.0359               &  & \textbf{skin}            & 0.2619               & 0.2597          & 0.276           & 0.2801          & 0.2864          & 0.2925               & 0.0306                \\
\textbf{agnews\_1}       & 0.5995               & 0.6258          & 0.6272          & 0.6305          & 0.6324          & 0.6327               & 0.0332               &  & \textbf{Stamps}          & 0.3182               & 0.3379          & 0.3457          & 0.351           & 0.3486          & 0.3468               & 0.0286                \\ 
\cmidrule[\heavyrulewidth]{1-8}\cmidrule[\heavyrulewidth]{10-17}
\multicolumn{1}{c}{}     & \multicolumn{1}{c}{} &                 &                 &                 &                 & \multicolumn{1}{c}{} &                      &  & \multicolumn{1}{c}{}     & \multicolumn{1}{c}{} &                 &                 &                 &                 & \multicolumn{1}{c}{} &                       \\ 
\cmidrule[\heavyrulewidth]{1-8}\cmidrule[\heavyrulewidth]{10-17}
\multicolumn{8}{c}{\textbf{(c) Student’s improvement compared to Teacher (HBOS) in terms of AUCROC }}                                                                     &  & \multicolumn{8}{c}{\textbf{(d) Student’s improvement compared to Teacher (HBOS) in terms of AP }}                                                                          \\ 
\cmidrule{1-8}\cmidrule{10-17}
\textbf{Datasets}        & \textbf{Teacher}     & \textbf{iter 2} & \textbf{iter 4} & \textbf{iter~6} & \textbf{iter~8} & \textbf{iter 10}     & \textbf{Improvement} &  & \textbf{Datasets}        & \textbf{Teacher}     & \textbf{iter 2} & \textbf{iter~4} & \textbf{iter~6} & \textbf{iter~8} & \textbf{iter~10}     & \textbf{Improvement}  \\ 
\cmidrule{1-8}\cmidrule{10-17}
\textbf{speech}          & 0.4673               & 0.5931          & 0.612           & 0.626           & 0.6299          & 0.633                & 0.1657               &  & \textbf{pendigits}       & 0.2805               & 0.3397          & 0.359           & 0.3671          & 0.3779          & 0.389                & 0.1085                \\
\textbf{Wilt}            & 0.3849               & 0.5111          & 0.5311          & 0.5492          & 0.5464          & 0.5426               & 0.1577               &  & \textbf{vowels}          & 0.0883               & 0.0865          & 0.1052          & 0.1254          & 0.1524          & 0.182                & 0.0936                \\
\textbf{vowels}          & 0.6726               & 0.7341          & 0.7732          & 0.7878          & 0.7987          & 0.8051               & 0.1325               &  & \textbf{Ionosphere}      & 0.4133               & 0.4516          & 0.5228          & 0.5313          & 0.5095          & 0.486                & 0.0727                \\
\textbf{mnist}           & 0.6141               & 0.6662          & 0.6623          & 0.6672          & 0.675           & 0.6779               & 0.0638               &  & \textbf{imgseg}          & 0.6105               & 0.644           & 0.6478          & 0.6476          & 0.6509          & 0.6538               & 0.0433                \\
\textbf{imgseg}          & 0.656                & 0.6945          & 0.7012          & 0.7032          & 0.7058          & 0.7096               & 0.0536               &  & \textbf{cardio}          & 0.4679               & 0.5132          & 0.5182          & 0.5134          & 0.5099          & 0.508                & 0.0401                \\
\textbf{optdigits}       & 0.8184               & 0.8715          & 0.8757          & 0.8777          & 0.8753          & 0.8714               & 0.053                &  & \textbf{mnist}           & 0.125                & 0.1479          & 0.1507          & 0.1524          & 0.1565          & 0.1588               & 0.0338                \\
\textbf{abalone}         & 0.4427               & 0.4701          & 0.477           & 0.4799          & 0.4836          & 0.4939               & 0.0511               &  & \textbf{Stamps}          & 0.3526               & 0.3783          & 0.3776          & 0.3818          & 0.384           & 0.3832               & 0.0307                \\
\textbf{annthyroid}      & 0.6431               & 0.661           & 0.6784          & 0.6918          & 0.6875          & 0.692                & 0.0489               &  & \textbf{Hepatitis}       & 0.3142               & 0.3007          & 0.3394          & 0.3264          & 0.365           & 0.3421               & 0.0278                \\
\textbf{vertebral}       & 0.2744               & 0.2259          & 0.2484          & 0.2731          & 0.2949          & 0.3208               & 0.0464               &  & \textbf{satimage-2}      & 0.826                & 0.8493          & 0.8483          & 0.8501          & 0.8522          & 0.8528               & 0.0268                \\
\textbf{Parkinson}       & 0.6799               & 0.6832          & 0.6861          & 0.6937          & 0.7112          & 0.7228               & 0.0429               &  & \textbf{Pima}            & 0.5463               & 0.5525          & 0.5645          & 0.5648          & 0.5644          & 0.564                & 0.0176                \\ 
\cmidrule[\heavyrulewidth]{1-8}\cmidrule[\heavyrulewidth]{10-17}
\multicolumn{1}{c}{}     & \multicolumn{1}{c}{} &                 &                 &                 &                 & \multicolumn{1}{c}{} &                      &  & \multicolumn{1}{c}{}     & \multicolumn{1}{c}{} &                 &                 &                 &                 & \multicolumn{1}{c}{} &                       \\ 
\cmidrule[\heavyrulewidth]{1-8}\cmidrule[\heavyrulewidth]{10-17}
\multicolumn{8}{c}{\textbf{(e) Student’s improvement compared to Teacher (LOF) in terms of AUCROC }}                                                                      &  & \multicolumn{8}{c}{\textbf{(f) Student’s improvement compared to Teacher (LOF) in terms of AP }}                                                                           \\ 
\cmidrule{1-8}\cmidrule{10-17}
\textbf{Datasets}        & \textbf{Teacher}     & \textbf{iter 2} & \textbf{iter 4} & \textbf{iter~6} & \textbf{iter~8} & \textbf{iter 10}     & \textbf{Improvement} &  & \textbf{Datasets}        & \textbf{Teacher}     & \textbf{iter 2} & \textbf{iter~4} & \textbf{iter~6} & \textbf{iter~8} & \textbf{iter~10}     & \textbf{Improvement}  \\ 
\cmidrule{1-8}\cmidrule{10-17}
\textbf{http}            & 0.3685               & 1               & 1               & 1               & 1               & 1                    & 0.6315               &  & \textbf{http}            & 0.0603               & 1               & 1               & 1               & 1               & 1                    & 0.9397                \\
\textbf{shuttle}         & 0.4886               & 0.9199          & 0.9244          & 0.9691          & 0.9537          & 0.9525               & 0.4638               &  & \textbf{shuttle}         & 0.0958               & 0.6814          & 0.7598          & 0.873           & 0.7902          & 0.7882               & 0.6924                \\
\textbf{satimage-2}      & 0.4702               & 0.5677          & 0.6909          & 0.7618          & 0.8402          & 0.9146               & 0.4444               &  & \textbf{optdigits}       & 0.0732               & 0.1114          & 0.1825          & 0.2627          & 0.3593          & 0.4551               & 0.3819                \\
\textbf{optdigits}       & 0.5819               & 0.8488          & 0.8884          & 0.9128          & 0.9318          & 0.9438               & 0.3619               &  & \textbf{satellite}       & 0.3746               & 0.6268          & 0.675           & 0.6887          & 0.7047          & 0.7117               & 0.3371                \\
\textbf{musk}            & 0.4586               & 0.5008          & 0.5584          & 0.6137          & 0.6848          & 0.7528               & 0.2942               &  & \textbf{WDBC}            & 0.1026               & 0.1757          & 0.2627          & 0.3202          & 0.3604          & 0.3754               & 0.2727                \\
\textbf{satellite}       & 0.5523               & 0.7405          & 0.7655          & 0.7749          & 0.7868          & 0.7902               & 0.238                &  & \textbf{FashionMNIST\_7} & 0.2485               & 0.3013          & 0.3345          & 0.3796          & 0.4325          & 0.4875               & 0.239                 \\
\textbf{speech}          & 0.5035               & 0.6552          & 0.6823          & 0.7019          & 0.7115          & 0.7182               & 0.2147               &  & \textbf{FashionMNIST\_1} & 0.1679               & 0.213           & 0.2372          & 0.2771          & 0.3291          & 0.3943               & 0.2263                \\
\textbf{FashionMNIST\_5} & 0.6806               & 0.7116          & 0.7807          & 0.8211          & 0.8572          & 0.8847               & 0.2041               &  & \textbf{FashionMNIST\_8} & 0.1246               & 0.1602          & 0.1917          & 0.2374          & 0.2996          & 0.3365               & 0.2119                \\
\textbf{FashionMNIST\_1} & 0.6669               & 0.7405          & 0.7768          & 0.8083          & 0.833           & 0.8566               & 0.1897               &  & \textbf{FashionMNIST\_5} & 0.1936               & 0.2157          & 0.2422          & 0.2776          & 0.3292          & 0.3971               & 0.2035                \\
\textbf{landsat}         & 0.5436               & 0.704           & 0.7161          & 0.713           & 0.713           & 0.7096               & 0.166                &  & \textbf{smtp}            & 0.0526               & 0.0556          & 0.3333          & 0.3333          & 0.25            & 0.25                 & 0.1974                \\ 
\cmidrule[\heavyrulewidth]{1-8}\cmidrule[\heavyrulewidth]{10-17}
\multicolumn{1}{c}{}     & \multicolumn{1}{c}{} &                 &                 &                 &                 & \multicolumn{1}{c}{} &                      &  & \multicolumn{1}{c}{}     & \multicolumn{1}{c}{} &                 &                 &                 &                 & \multicolumn{1}{c}{} &                       \\ 
\cmidrule[\heavyrulewidth]{1-8}\cmidrule[\heavyrulewidth]{10-17}
\multicolumn{8}{c}{\textbf{(g) Student’s improvement compared to Teacher (KNN) in terms of AUCROC }}                                                                      &  & \multicolumn{8}{c}{\textbf{(h) Student’s improvement compared to Teacher (KNN) in terms of AP }}                                                                           \\ 
\cmidrule{1-8}\cmidrule{10-17}
\textbf{Datasets}        & \textbf{Teacher}     & \textbf{iter 2} & \textbf{iter 4} & \textbf{iter~6} & \textbf{iter~8} & \textbf{iter 10}     & \textbf{Improvement} &  & \textbf{Datasets}        & \textbf{Teacher}     & \textbf{iter 2} & \textbf{iter~4} & \textbf{iter~6} & \textbf{iter~8} & \textbf{iter~10}     & \textbf{Improvement}  \\ 
\cmidrule{1-8}\cmidrule{10-17}
\textbf{Stamps}          & 0.6587               & 0.773           & 0.8458          & 0.8863          & 0.8876          & 0.8851               & 0.2264               &  & \textbf{shuttle}         & 0.1558               & 0.9055          & 0.9203          & 0.8229          & 0.7425          & 0.7379               & 0.5822                \\
\textbf{SpamBase}        & 0.5086               & 0.6249          & 0.6675          & 0.692           & 0.7087          & 0.7119               & 0.2033               &  & \textbf{satimage-2}      & 0.3294               & 0.4703          & 0.5803          & 0.6749          & 0.8082          & 0.8873               & 0.5579                \\
\textbf{pendigits}       & 0.7133               & 0.8409          & 0.8484          & 0.8691          & 0.8861          & 0.9047               & 0.1914               &  & \textbf{satellite}       & 0.5041               & 0.7098          & 0.7306          & 0.7448          & 0.7609          & 0.7683               & 0.2642                \\
\textbf{musk}            & 0.6845               & 0.775           & 0.7961          & 0.8153          & 0.8377          & 0.8551               & 0.1706               &  & \textbf{SpamBase}        & 0.3967               & 0.4643          & 0.5138          & 0.5479          & 0.5746          & 0.5815               & 0.1848                \\
\textbf{shuttle}         & 0.6618               & 0.9908          & 0.9903          & 0.9365          & 0.8425          & 0.8134               & 0.1516               &  & \textbf{WPBC}            & 0.232                & 0.2343          & 0.2788          & 0.3481          & 0.3952          & 0.4123               & 0.1803                \\
\textbf{speech}          & 0.4791               & 0.5861          & 0.6065          & 0.6213          & 0.626           & 0.6289               & 0.1498               &  & \textbf{Stamps}          & 0.1598               & 0.1868          & 0.2292          & 0.2873          & 0.322           & 0.3343               & 0.1745                \\
\textbf{WPBC}            & 0.4643               & 0.4833          & 0.5247          & 0.5555          & 0.589           & 0.6088               & 0.1445               &  & \textbf{musk}            & 0.0897               & 0.0805          & 0.0969          & 0.132           & 0.2204          & 0.253                & 0.1633                \\
\textbf{satellite}       & 0.6536               & 0.7617          & 0.7724          & 0.7788          & 0.7889          & 0.7932               & 0.1396               &  & \textbf{wine}            & 0.0789               & 0.1071          & 0.1403          & 0.2368          & 0.244           & 0.2422               & 0.1633                \\
\textbf{WBC}             & 0.8503               & 0.9611          & 0.9688          & 0.9756          & 0.9819          & 0.9736               & 0.1234               &  & \textbf{landsat}         & 0.2511               & 0.3578          & 0.3689          & 0.3738          & 0.38            & 0.3839               & 0.1328                \\
\textbf{WDBC}            & 0.7211               & 0.7883          & 0.8263          & 0.8357          & 0.8406          & 0.839                & 0.1179               &  & \textbf{annthyroid}      & 0.1742               & 0.1874          & 0.2024          & 0.2207          & 0.251           & 0.3014               & 0.1272                \\
\cmidrule[\heavyrulewidth]{1-8}\cmidrule[\heavyrulewidth]{10-17}
\end{tabular}}
\end{table*}

\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{pictures/box_aucroc.png}
\caption{Boxplot of AUCROC on 84 datasets}
\label{fig:y equals x}
\end{subfigure}
\begin{subfigure}[b]{0.9\linewidth}
\centering
\includegraphics[width=\textwidth]{pictures/box_ap.png}
\caption{Boxplot of AP on 84 datasets}
\label{fig:three sin x}
\end{subfigure}
\caption{
Comparison between booster's performance and target UAD's performance in terms of AUCROC and AP over 84 datasets.
Higher AUCROC/AP is better.
}
\label{fig:box overall}
\end{figure*}

==> sections/notes.tex <==
\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

==> sections/preliminaries.tex <==
\subsection{Preliminaries}
\label{sec:preliminaries}
We will first formally define the definitions of basic notations.
Let $d$ denote the number of input features, $n$ as the number of training samples, $l$ as the number of test samples, $\textbf{X} = \{\textbf{x}_1,...,\textbf{x}_n\} \in \mathbb{R}^{n\times d}$ as training set, $\textbf{X}_{\rm test} \in \mathbb{R}^{l\times d}$ as test set, $\textbf{Y}_{\rm test} \in \mathbb{R}^{l\times 1}$ as test ground truth which is only used for evaluation.
As mentioned above, we use teacher model: $M_{\rm teacher}$ to represent the unsupervised model and student model: $M_{\rm student}$ to represent approximator.
Here, the student model is a cascade model that should be trained for numerous iterations (please see Section~\ref{sec:correct mechanism} for more details), let $N$ denote the total number of iterations, $\textbf{Y}: \{\textbf{y}_{i}\}_{i=1,2,...,N}$ as pseudo labels, where $\textbf{y}_i$ is used as training label in $i$-th iteration. 

\begin{table}[t]
\caption{Definitions of basic notations}
\centering
\begin{tabular}{c|c} 
\toprule
\textbf{Notation} & \textbf{Definition}         \\ 
\midrule
$d$                 & Number of input dimensions  \\ 
\hline
$n$                 & Number of training samples  \\ 
\hline
$l$                 & Number of test samples      \\ 
\hline
$\textbf{X} \in \mathbb{R}^{n\times d}$                 & Training set                \\ 
\hline
$\textbf{X}_{\rm test} \in \mathbb{R}^{l\times d}$           & Test test                   \\ 
\hline
$\textbf{Y}_{\rm test} \in \mathbb{R}^{l\times 1}$           & Test ground truth           \\ 
\hline
$M_{\rm teacher}$        & Teacher model               \\ 
\hline
$M_{\rm student}$        & Student model               \\
\hline
$N$        & Number of total iterations               \\
\hline
$\textbf{Y}: \{\textbf{y}_{i}\}_{i=1,2,...,N}$        & Collection of all iterations' pseudo labels              \\
\hline
$\textbf{P}_{\rm teacher}$        & Output of teacher model              \\
\hline
$\textbf{P}_{\rm student}$        & Output of student model              \\
\bottomrule
\end{tabular}
\end{table}
For unsupervised AD, the goal is to train an anomaly detection model on training set without true labels to predict anomaly score on test set, where anomaly score is a continues value $\in [0,1]$ and higher score indicates higher probability that a sample is an anomaly.
Here, the teacher model: $M_{\rm teacher}$ is trained on $\textbf{X}$ to return anomaly score $\textbf{P}_{\rm teacher}:= M_{\rm teacher}(\textbf{X}) \in \mathbb{R}^{n\times 1}$, which is used as the initial pseudo label $\textbf{y}_1$.
Let $\mathcal{L}$ be the loss function.
Then during each iteration, we aim to minimize: $\mathcal{L}(M_{\rm student}(\textbf{X}), \textbf{y}_i)$.
Finally, we need to predict on $\textbf{X}_{\rm test}$, to return $M_{\rm student}(\textbf{X}_{\rm test})$ for evaluation.

